GameSWE: Evaluating Coding Agents in Live Game Runtimes

Coding agents are increasingly evaluated on repository-level tasks, where a change is judged by the repository's own tests. Yet much software runs inside a live host program, where correctness depends on runtime state, lifecycle events, and third-party components loaded alongside it. We introduce GameSWE, a benchmark of 150 repair and construction tasks built from open-source mods for 12 popular games across five programming languages. Each submission is compiled, loaded into the real game or its dedicated server together with the pinned third-party mods it depends on, and judged by fail-to-pass and pass-to-pass tests executed in the live runtime, without mocks or LLM judges. Across seven frontier and open-weight models, the best agent resolves 69.0% of tasks while three models remain at or below 25.0%, and even the best agent's per-game rate ranges from 40.0% to 93.3%. Our analysis shows that 70.0% of unresolved attempts end with the agent submitting its work as complete, and in at least 31.0% the agent reports that its own checks pass, yet the submission fails in the runtime, with failures concentrated at the boundary between code and host: interfaces the ecosystem does not provide, host conventions beyond the code, and logic not connected to the game's lifecycle. GameSWE provides a reproducible testbed for coding agents whose code must work where it runs.

==> packages.tex <==
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{mathtools}                %
\RequirePackage{bm}                       %
\RequirePackage{mathpazo}

\RequirePackage{microtype}
\RequirePackage{anyfontsize}
\RequirePackage{titlesec}
\RequirePackage{tocloft}
\RequirePackage[defaultsans]{lato}        %

\RequirePackage{xcolor}
\RequirePackage{colortbl}
\definecolor{gblue}{HTML}{1A73E8}     %
\definecolor{gred}{HTML}{D93025}      %
\definecolor{gyellow}{HTML}{E37400}   %
\definecolor{ggreen}{HTML}{1E8E3E}    %
\definecolor{gpurple}{HTML}{9334E6}   %
\definecolor{ggrey}{HTML}{5F6368}     %
\colorlet{linkcol}{black}

\RequirePackage{graphicx}
\RequirePackage{wrapfig}
\RequirePackage{adjustbox}
\RequirePackage{tikz}                     %

\RequirePackage[labelsep=colon]{caption}
\RequirePackage{subcaption}               %

\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{makecell}

\RequirePackage{geometry}
\RequirePackage{fancyhdr}
\RequirePackage{authblk}
\RequirePackage{enumitem}
\RequirePackage{tcolorbox}

\RequirePackage{verbatim}
\RequirePackage{pifont}

\RequirePackage[ruled,vlined,linesnumbered]{algorithm2e}

\RequirePackage[numbers,sort&compress]{natbib}

\RequirePackage[colorlinks=true,allcolors=linkcol]{hyperref}
\RequirePackage[capitalize,noabbrev]{cleveref} %

